What the Vec? Towards Probabilistically Grounded Embeddings

Word2Vec (W2V) and GloVe are popular, fast and efficient word embedding algorithms. Their embeddings are widely used and perform well on a variety of natural language processing tasks. Moreover, W2V has recently been adopted in the field of graph embedding, where it underpins several leading algorithms. However, despite their ubiquity and relatively simple model architecture, a theoretical understanding of what the embedding parameters of W2V and GloVe learn and why that is useful in downstream tasks has been lacking. We show that different interactions between PMI vectors reflect semantic word relationships, such as similarity and paraphrasing, that are encoded in low dimensional word embeddings under a suitable projection, theoretically explaining why embeddings of W2V and GloVe work. As a consequence, we also reveal an interesting mathematical interconnection between the considered semantic relationships themselves.

==> sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}

Pipeline of W2V : 
\begin{itemize}
    \item Extract statistics
    \item Empirical estimates of probability parameters (nothing done to de-noise)
    \item Projection to lower dimension, geometry subject to loss function - lost dimensions are those of least variance - since PMI, those of least information..?
    \item Downstream task - how embeddings are compared/combined depends on what is learned / how it's encoded.
\end{itemize}


\subsection{other}

Different properties can be used:
\begin{itemize}
    \item \textbf{intrinsic} features: letters in the word, phonetic sound, thesaurus words; or
    \item \textbf{extrinsic} (or relative) features: statistics of co-occurrences
\end{itemize}
The main difference is that the first might be turned into a representation by distilling commonalities, or underlying latent features, e.g. by dimensionality reduction; the latter require a binary comparison, requiring an interaction to be defined, e.g. inner product, distance.



\subsection{What is an embedding?}

The problem of `embedding' runs deep: we seek a isomorphism of the set (in a mathematical sense) of words $w\in\mathcal{E}$ to points in $\mathbb{R}^d$. However, the operation(s) to be preserved are unclear and are not obviously expressible in terms of other $w$, i.e. $\mathcal{E}$ cannot be considered a group, ring etc and use of formal rigorous representation methods (eg see group character) do not (currently) seem readily applicable.

\begin{itemize}
    \item an encoding of pertinent information about data points (intrinsic), or  relationships between them (extrinsic), or both.
    % 
    \item what is stored and how determines what we want back and how we want it.
    % 
    \item one-hot encodings suffice to uniquely identify objects in a set
    % 
    \item if data points form a mathematical structure (e.g. group, ring), then relationships might be defined in terms of other elements and an embedding or representation might map the entire structure \textit{isomorphically} (e.g. characters)
    % 
    \item embeddings that capture or encode intrinsic properties, e.g. dimensionality reduction, preserve certain dimensional properties (or linear combinations thereof) but lose any information in others. The encoding can be used by projection back to the original dimensionality to approximate or de-noise the original data, or certain comparisons might be made in the lower dimensional space.
    % 
    \item relationships however may be lost or obscured in the lower dimensionality, depending on the nature of the relationship and the encoding method, e.g. if relationships are encoded by Euclidean distance, they are retained under translation (e.g. by shift term!?), whereas relationship encoded in the dot product of vectors from the origin are distorted (although are fully retrievable).
    % 
    \item \textit{Unsupervised} embedding is ill-posed since the information to be captured and the method by which we want to retrieve it are both unknown. For example, the manifestation of analogies as additive combinations of embeddings relies on a logarithm within the embedding process, whereas if embeddings are only to be `plugged in' to a downstream model, perhaps such a property is superfluous, perhaps even detrimental in the sense that it is not present in an optimal encoding (should such a concept exist) that, for example, needed to preserve underlying probability parameters \textit{linearly}. Unsupervised $\approx$ human-in-loop supervised??
    % 
    \item in general, however it is achieved, so long as information is captured then it can be retrieved. However, certain methods may be more convenient or fit better with downstream tasks or require less computation. In particular it may help to know what is stored and how it is stored if we are to make best use of it. This is often not the case.
\end{itemize}

